The evolving relation between star-formation rate and stellar mass in the VIDEO Survey since $z=3$

We investigate the star-formation rate (SFR) and stellar mass ($M_*$) relation of a star-forming (SF) galaxy sample in the XMM-LSS field to $z\sim 3.0$ using the near-infrared data from the VISTA Deep Extragalactic Observations (VIDEO) survey. Combining VIDEO with broad-band photometry, we use the SED fitting algorithm CIGALE to derive SFRs and $M_*$ and have adapted it to account for the full photometric redshift PDF uncertainty. Applying a SF selection using the D4000 index, we find evidence for strong evolution in the normalisation of the SFR-$M_*$ relation out to $z\sim 3$ and a roughly constant slope of (SFR $\propto M_*^{\alpha}$) $\alpha=0.69\pm0.02$ to $z\sim 1.7$. We find this increases close to unity toward $z\sim2.65$. Alternatively, if we apply a colour selection, we find a distinct turnover in the SFR-$M_*$ relation between $0.7\lesssim z\lesssim2.0$ at the high mass end, and suggest that this is due to an increased contamination from passive galaxies. We find evolution of the specific SFR $\propto(1+z)^{2.60}$ at $\log(M_*)\sim$10.5, out to $z\lesssim2.4$ with an observed flattening beyond $z\sim$ 2 with increased stellar mass. Comparing to a range of simulations we find the analytical scaling relation approaches, that invoke an equilibrium model, a good fit to our data, suggesting that a continual smooth accretion regulated by continual outflows may be a key driver in the overall growth of SFGs.

==> tab_fig11_fits.tex <==
\begin{table}
\caption{Details of the properties of the various constraints compared in this  work. }
\label{tab:fig11fits}
\centering
\scriptsize
\begin{tabular}{c c c c c c c c c }
&  \multicolumn{2}{c}{uncalibrated} &  \multicolumn{2}{c}{calibrated} \\
&     \multicolumn{2}{c}{$\overbrace{\rule{2cm}{0pt}}$} &  \multicolumn{2}{c}{$\overbrace{\rule{2cm}{0pt}}$} \\
Work    &  $\alpha$ & $\beta$   &  $\alpha$ & $\beta$ \\

\hline\hline
$0.1<z<0.8$ \\ 
\citet{Dunne:2009MNRAS.394....3D}     	& 0.83 $\pm$ 0.01  	& -7.92 $\pm$ 0.13  	& 0.83 $\pm$ 0.01 	& -7.83 $\pm$ 0.13		\\
\citet{Noeske:2007ApJ...660L..47N} 		& 0.67 $\pm$ 0.08 	& -6.19 $\pm$ 0.78 	& 0.67 $\pm$ 0.08 	& -6.00 $\pm$ 0.78		\\
\citet{Oliver2010MNRAS.405.2279O} 	& 0.73 $\pm$ 0.05 	& -7.02 $\pm$ 0.55 	& 0.73 $\pm$ 0.05	& -6.86 $\pm$  0.55   	 \\
\citet{Santini2009AA...504..751S} 		& 0.70 $\pm$ 0.14 	& -6.33 $\pm$ 1.54   & 0.70 $\pm$ 0.14 	& -6.27 $\pm$ 1.54	\\ \\

$0.8<z<1.2$ \\ 
\citet{Dunne:2009MNRAS.394....3D}         & 0.83 $\pm$ 0.05 	& -7.38 $\pm$ 0.53    & 0.83 $\pm$  0.05 	& ?7.39 $\pm$  0.53      \\
\citet{Elbaz2007AA...468...33E} 		& 0.90 			& -8.14			 & 0.90			& -8.06			\\\\

$1.9<z<2.1$ \\ 
\citet{daddi07}  						 & 0.90 			& -7.6 			& 0.90			& -7.52		\\ 
\citet{Dunne:2009MNRAS.394....3D}          & 0.88 $\pm$ 0.03  	& -7.21 $\pm$  0.37 & 0.88  $\pm$ 0.03    & -7.36 $\pm$ 0.37 \\
\citet{Pannella2009ApJ...698L.116P}          & 0.95 $\pm$ 0.07	& -8.30   			& \\	
\citet{Reddy2012ApJ...754...25R}               & 0.97 $\pm$ 0.05   & -8.28 $\pm$ 1.28   & \\
\citet{Rodighiero2011ApJ...739L..40R}  	 & 0.79 			& -6.42			& \\
\citet{Zahid2012ApJ...757...54Z}             \\\\


  	

\hline
\end{tabular}
\end{table}

